Approximate Gomory-Hu Tree Is Faster Than $n-1$ Max-Flows

The Gomory-Hu tree or cut tree (Gomory and Hu, 1961) is a classic data structure for reporting $(s,t)$ mincuts (and by duality, the values of $(s,t)$ maxflows) for all pairs of vertices $s$ and $t$ in an undirected graph. Gomory and Hu showed that it can be computed using $n-1$ exact maxflow computations. Surprisingly, this remains the best algorithm for Gomory-Hu trees more than 50 years later, *even for approximate mincuts*. In this paper, we break this longstanding barrier and give an algorithm for computing a $(1+\epsilon)$-approximate Gomory-Hu tree using $\text{polylog}(n)$ maxflow computations. Specifically, we obtain the runtime bounds we describe below. We obtain a randomized (Monte Carlo) algorithm for undirected, weighted graphs that runs in $\tilde O(m + n^{3/2})$ time and returns a $(1+\epsilon)$-approximate Gomory-Hu tree algorithm w.h.p. Previously, the best running time known was $\tilde O(n^{5/2})$, which is obtained by running Gomory and Hu's original algorithm on a cut sparsifier of the graph. Next, we obtain a randomized (Monte Carlo) algorithm for undirected, unweighted graphs that runs in $m^{4/3+o(1)}$ time and returns a $(1+\epsilon)$-approximate Gomory-Hu tree algorithm w.h.p. This improves on our first result for sparse graphs, namely $m = o(n^{9/8})$. Previously, the best running time known for unweighted graphs was $\tilde O(mn)$ for an exact Gomory-Hu tree (Bhalgat et al., STOC 2007); no better result was known if approximations are allowed. As a consequence of our Gomory-Hu tree algorithms, we also solve the $(1+\epsilon)$-approximate all pairs mincut and single source mincut problems in the same time bounds. (These problems are simpler in that the goal is to only return the $(s,t)$ mincut values, and not the mincuts.) This improves on the recent algorithm for these problems in $\tilde O(n^2)$ time due to Abboud et al. (FOCS 2020).

==> minimal.tex <==
This section proves \thm{rooted}, restated below.
\Rooted*

Let $\e>0$ be a small enough weight, and let $G'$ be the graph $G$ with an additional edge $(r,v)$ of weight $\e$ added for each $v\in V\sm\{r\}$. (If the edge $(r,v)$ already exists in $G$, then increase its weight by $\e$ instead.) If $\e>0$ is small enough, then for all $t\in V\sm\{r\}$ and $S\s V$, if $\pt_{G'}S$ is an $(r,t)$-mincut in $G'$, then $\pt_GS$ is an $(r,t)$-mincut in $G$.

Let $(T',f)$ be a Gomory-Hu Steiner tree for $G'$. We claim that it is essentially a minimal Gomory-Hu Steiner tree for $G$, except that its edge weights need to be recomputed as mincuts in $G$ and not $G'$. More formally, let $T$ be the tree $T'$ with the following edge re-weighting: for each edge $(u,v)$ in $T$, take a connected component $U'$ of $T-(u,v)$ and reset the edge weight of $(u,v)$ to be $w(\pt_Gf\inv(U'))$ and not $w(\pt_{G'}f\inv(U'))$. We now claim that $(T,f)$ is a minimal Steiner Gomory-Hu tree for $G$.

We first show that $(T,f)$ is a Gomory-Hu Steiner tree for $G$. Fix $s,t\in U$, let $(u,v)$ be the minimum-weight edge on the $s-t$ path in $T'$, and let $U'$ be the vertices of the connected component of $T'-(u,v)$ containing $s$. Since $(T',f)$ is a Gomory-Hu Steiner tree for $G'$, we have that $\pt_{G'}f\inv(U')$ is an $(s,t)$-mincut in $G'$. If $\e>0$ is small enough, then by our argument from before, $\pt_Gf\inv(U')$ is also an $(s,t)$-mincut in $G$. By our edge re-weighting of $T$, the edge $(u,v)$ has the correct weight. Moreover, $(u,v)$ is the minimum-weight edge on the $s-t$ path in $T$, since a smaller weight edge would contradict the fact that $\pt_Gf\inv(U')$ is an $(s,t)$-mincut.

We now show the additional property $(*)$ that makes $(T,f)$ a minimal Gomory-Hu Steiner tree. Fix $t\in U\sm\{r\}$, and let $(u,v)$ and $U'$ be defined as in $(*)$, i.e., $(u,v)$ is the minimum-weight edge $(u,v)$ on the $r-t$ path that is closest to $t$, and $U'$ is the vertices of the connected component of $T-(u,v)$ containing $r$. Since $(T,f)$ is a Gomory-Hu Steiner tree for $G$, we have that $\pt_Gf\inv(U')$ is an $(r,t)$-mincut of value $w_T(u,v)$. Suppose for contradiction that $\pt_Gf\inv(U')$ is not a \emph{minimal} $(r,t)$-mincut. Then, there exists $S\subsetneq f\inv(U')$ such that $\pt S$ is also an $(r,t)$-mincut. By construction of $G'$, $w(\pt_{G'}S)=w(\pt_GS)+|S|\e$ and $w(\pt_{G'}f\inv(U')) = w(\pt_Gf\inv(U'))+|f\inv(U')|\e$. We have $w(\pt_GS)=w(\pt_Gf\inv(U'))$ and $|S|<|f\inv(U')|$, so $w(\pt_{G'}S)<w(\pt_{G'}f\inv(U'))$. In other words, $f\inv(U')$ is not an $(r,t)$-mincut in $G'$, contradicting the fact that $(T',f)$ is a Gomory-Hu Steiner tree for $G'$. Therefore, property $(*)$ is satisfied, concluding the proof.






% THIS PROOF IS MORALLY CORRECT BUT IT'S BUGGY, IGNORE AND PROVE SIMPLER VARIANT (SLIGHTLY WEAKER BUT ENOUGH FOR OUR PURPOSES)
\iffalse

Consider a Gomory-Hu Steiner tree $T$ on $U$ with the following special property. Root the tree $T$ at $s$. For each vertex $v\in U$, let $U_v\s U$ denote the vertices in the subtree rooted at $v$. Then, the multiset $M(T,f)=\{ |f\inv(U_v)| : v\in U\}$, once sorted from largest to smallest, is lexicographically minimal among all valid Gomory-Hu trees on $U$ rooted at $s$. Assuming this special condition, we claim that $T$ must be a minimal Gomory-Hu Steiner tree rooted at $s$.

\alert{$s$ is overloaded. Please use a different notation to avoid overloading.}

Suppose not, and let $s,t,u,v\in U$ be vertices violating $(*)$ in Definition~\ref{defn:minimalGH}, chosen so that the depth of $t$ in the rooted tree $T$ is the maximum possible among all such violating pairs. Consider the minimal $(s,t)$-mincut and let $S$ be the side containing $s$, so that $S\subsetneq f\inv(U_u)$.

\alert{DP: A figure will help showing the relative positions of $s, t, u, v$ and the sets $U_u, S$, etc. will help here.}

\BCL\clml{Us}
For any $s'\in U_u\sm \{u\}$, we must have either $f\inv(U_{s'})\s S$ or $f\inv(U_{s'})\cap S=\emptyset$.
\ECL
\BP
Suppose the statement fails for some $s'\in U_u\sm u$. Let $t'\in U_u$ be the parent of $s'$.

Suppose first that $s'\in S$. Since $\pt(S\cup f\inv(U_{s'}))$ is an $(s,t)$-cut and $\pt(S\cap f\inv(U_{s'}))$ is an $(s',t')$-cut, by the submodularity of cuts,
\BAL
\mincut_G(s,t)+\mincut_G(s',t')&=w(\pt S)+w(\pt f\inv(U_{s'})) 
\\&\ge w(\pt(S\cup f\inv(U_{s'}))) + w(\pt(S\cap f\inv(U_{s'}))) 
\\&\ge \mincut_G(s,t) + \mincut_G(s',t').
\EAL
So, in particular, $\pt(S\cap f\inv(U_{s'})) \subsetneq f\inv(U_{s'})$ is an $(s',t')$-mincut, and the pair $(s',t')$ also violates $(*)$. Since $t'$ is a descendant of $t$, this contradicts our initial choice of $t$ whose depth is maximum possible. 

Suppose next that $s'\notin S$. Since $\pt(S\sm f\inv(U_{s'}))$ is an $(s,t)$-cut \alert{DP: Why? Can't you have $s\in U_{s'}\cap S$?} and $\pt(f\inv(U_{s'})\sm S)$ is an $(s',t')$-cut, by the submodularity of cuts,
\BAL
\mincut_G(s,t)+\mincut_G(s',t')&=w(\pt S)+w(\pt f\inv(U_{s'})) 
\\&\ge w(\pt(S\sm f\inv(U_{s'}))) + w(\pt(f\inv(U_{s'})\sm S)) 
\\&\ge \mincut_G(s,t) + \mincut_G(s',t').
\EAL
So in particular, $\pt(f\inv(U_{s'})\sm S)\subsetneq f\inv(U_{s'})$ is an $(s',t')$-mincut, and we obtain the same contradiction. 
\EP

\BCL\clml{inS}
For any $s'\in U_u$, we must have $s'\in S$.
\ECL
\BP
By construction, every edge in $T$ on the path $P$ from $s$ to $u$ has weight greater than $\mincut_G(s,t)$. If $s'\notin S$ for some vertex $s'$ on the path $P$, then $S$ is a $(s,s')$-cut, so there must be an edge with weight at most $w(\pt S)=\mincut_G(s,t)$ on the path from $s$ to $s'$, a contradiction. Suppose now that some vertex $s'\in U_u$ not on the path $P$ satisfies $s'\notin S$. We can choose $s'$ whose depth in the rooted tree $T$ is minimum possible. Let $t'$ be the parent of $s'$, so that $t'\in S$. Since $S$ is an $(s',t')$-cut, we must have 
\[ w(\pt f\inv(U_{s'}))=\mincut(s',t')\le w(\pt S) = \mincut(s,t) ,\]
so $w_T(s',t')\le w_T(s,t)$. 
We modify the tree $T$ into $T'$ as follows. Remove the edge $(s',t')$, and add the edge $(s',t)$ of the same weight $w(\pt f\inv(U_{s'}))$. We claim that $(T',f)$ is still a Gomory-Hu Steiner tree, which can be checked on a case-by-base basis, most of which are trivial and therefore omitted. The only nontrivial case is when the minimum weight edge is $(u,t)$, because the only vertex whose subtree has a different set of vertices between $T$ and $T'$ is $u$, whose subtree in $T$ is $U_u\sm U_{s'}$. \alert{Presumably, this is a typo and you actually wanted to write $T'$ instead of $T$. But, even so, why is the statement true? Doesn't $t'$ for instance that a different set if descendants between the two trees?} By \clm{Us}, $f\inv(U_{s'})\cap S=\emptyset$, and by the submodularity of cuts,
\BAL
\mincut_G(s,t)+\mincut_G(s',t')&=w(\pt f\inv(U_u))+w(\pt f\inv(U_{s'})) 
\\&\ge w(\pt(f\inv(U_u)\sm f\inv(U_{s'}))) + w(\pt(f\inv(U_{s'})\sm f\inv(U_u))) 
\\&\ge \mincut_G(s,t) + \mincut_G(s',t').
\EAL
\alert{Isn't $U_{s'}\subset U_u$? How can we uncross in that case?}
So, $\pt (f\inv(U_u)\sm f\inv(U_s)) = \pt f\inv(U_u\sm U_s)$ is an $(s,t)$-mincut.

Therefore, $(T',f)$ is a Gomory-Hu Steiner tree.
Furthermore, the multiset $M(T',f)$, once sorted from largest to smallest, is lexicographically smaller. This contradicts the choice of $(T,f)$.
\EP

Combining \Cref{clm:Us,clm:inS}, we conclude that $u\in S$ and for all $s'\in U_u\sm u$, we must have $f\inv(U_{s'})\s S$. Since $S\subsetneq f\inv(U_u)$ by assumption, the only remaining possibility is $S\cap f\inv(u) \subsetneq f\inv(u)$. We modify $f$ into $f'$ as follows: we keep $f'(v)=f(v)$ for all $v\in V\sm(f\inv(u)\sm S)$, but we modify $f'(v)=t$ for all $v\in f\inv(u)\sm S$ (while $f(v)=u$). \alert{DP: $v$ has a specific meaning as the parent of $u$; perhaps use a different letter here?} Then, $f\inv(U_u)=S$, and it is easy to verify that $(T,f')$ is a Gomory-Hu Steiner tree whose multiset $M(T,f')$, once sorted, is lexicographically smaller. This contradicts the choice of $(T,f)$. \alert{Why is $(T, f')$ a Gomory-Hu Steiner tree? This seems to change the identity of all $U_x$ where $x$ is between $u$ and $t$ in $T$.}

Thus, the assumption $S\subsetneq f\inv(U_u)$ is false to begin with, concluding the proof of \thm{rooted}.

\fi



==> prelim.tex <==
\alert{DP: We need to merge in these prelims into the previous section, perhaps into techniques?} \textcolor{blue}{JL: sure, feel free to reorganize definitions and prelims}

\BD[Minimum isolating cuts]
Consider a weighted, undirected graph $G=(V,E)$ and a subset $R\s V$ ($|R|\ge2$). The \emph{minimum isolating cuts} for $R$ is a collection of sets $\{S_v:v\in R\}$ such that for each vertex $v\in R$, the set $S_v$ satisfies $S_v\cap R=\{v\}$ and has the minimum value of $w(\pt S'_v)$ over all sets $S'_v$ satisfying $S'_v\cap R=\{v\}$.
\ED

%\alert{DP: In the above definition, should we also mention that sets $S_v$ must be disjoint? At the moment, this is in the next lemma. Would putting it in the definition might make life a bit easier in terms of just having to refer to the definition when invoking this property?}

\BL
Fix a subset $R\s V$ ($|R|\ge2$). There is an algorithm that computes the minimum isolating cuts $\{S_v:v\in R\}$ for $R$ using $O(\log|R|)$ calls to $s-t$ max-flow on weighted graphs of $O(n)$ vertices and $O(m)$ edges, and takes $\tO(m)$ deterministic time outside of the max-flow calls. If the original graph $G$ is unweighted, then the inputs to the max-flow calls are also unweighted. Moreover, the sets $\{S_v:v\in R\}$ are disjoint.
\EL

%\alert{DP: In the above lemma, should we use $\lceil \lg |R|\rceil$ or $O(\log |R|)$? It depends on whether the constant is important to preserve.}

\BD[Single-source min-cut]
In the \emph{single-source min-cut} (SSMC) problem, the input is an undirected graph $G=(V,E)$ and a source vertex $s\in V$, and we need to output a $(s,v)$-mincut for each $v\in V\sm \{s\}$. In the \emph{$(1+\e)$-approximate SSMC} problem, the input is the same, and we need to output a $(1+\e)$-approximate $(s,v)$-mincut for each $v\in V\sm \{s\}$.
\ED


\BD[Gomory-Hu Steiner tree]
Given a graph $G=(V,E)$ and a set of terminals $U\s V$, the Gomory-Hu Steiner tree is a weighted tree $T$ on the vertices $U$, together with a function $f:V\to U$, such that
 \BI
 \im For all $s,t\in U$, consider the minimum-weight edge $(u,v)$ on the unique $s-t$ path in $T$. Let $U'$ be the vertices of the connected component of $T-(u,v)$ containing $s$.
Then, the set $f\inv(U')\s V$ is an $(s,t)$-mincut, and its value is $w_T(u,v)$.
 \EI
\ED

\BD[Approximate Gomory-Hu Steiner tree]
Given a graph $G=(V,E)$ and a set of terminals $U\s V$, the $(1+\e)$-approximate Gomory-Hu Steiner tree is a weighted tree $T$ on the vertices $U$, together with a function $f:V\to U$, such that
 \BI
 \im For all $s,t\in U$, consider the minimum-weight edge $(u,v)$ on the unique $s-t$ path in $T$. Let $U'$ be the vertices of the connected component of $T-(u,v)$ containing $s$.
Then, the set $f\inv(U')\s V$ is a $(1+\e)$-approximate $(s,t)$-mincut, and its value is $w_T(u,v)$.
 \EI
\ED

\BD[Rooted minimal Gomory-Hu Steiner tree]\label{defn:minimalGH}
Given a graph $G=(V,E)$ and a set of terminals $U\s V$, a rooted minimal Gomory-Hu Steiner tree is a Gomory-Hu Steiner tree on $U$, rooted at some vertex $r\in U$, with the following additional property:
 \BI
% MORE GENERAL BUT HARDER TO PROVE, SO WE SKIPPED -> \im[$(*)$] For all $s,t\in U$ where $s$ is a descendant of $t$ in the rooted tree $T$, consider the minimum-weight edge $(u,v)$ on the unique $s-t$ path in $T$; if there are multiple minimum weight edges, let $(u, v)$ denote the one that is {\em closest to $s$}. Let $U'$ be the vertices of the connected component of $T-(u,v)$ containing $s$.
 \im[$(*)$] For all $t\in U\sm\{r\}$, consider the minimum-weight edge $(u,v)$ on the unique $r-t$ path in $T$; if there are multiple minimum weight edges, let $(u, v)$ denote the one that is {\em closest to $t$}. Let $U'$ be the vertices of the connected component of $T-(u,v)$ containing $r$.
Then, $\pt_Gf\inv(U')\s V$ is a \emph{minimal} $(r,t)$-mincut, and its value is $w_T(u,v)$.
 \EI
\ED

The following theorem, proved in the appendix, establishes the existence of a rooted minimal Gomory-Hu Steiner tree rooted at any given vertex.

\begin{restatable}{theorem}{Rooted}\thml{rooted}
For any graph $G=(V,E)$, terminals $U\s V$, and root $r\in U$, there exists a rooted minimal Gomory-Hu Steiner tree rooted at $r$.
\end{restatable}

\eat{

\subsection{Our Results}

\begin{restatable}{theorem}{ApproxU}\thml{approx-u}
Let $G$ be an unweighted, undirected graph. There is a randomized algorithm that w.h.p., outputs a $(1+\e)$-approximate Gomory-Hu Steiner tree and runs in $\tO(m)$ time plus calls to max-flow on instances with a total of $\tO(n\e\inv)$ vertices and $\tO(m\e\inv)$ edges. Using the $m^{4/3+o(1)}$-time max-flow algorithm for unweighted graphs of Liu~and~Sidford, the algorithm runs in $m^{4/3+o(1)}\e\inv$ time.
\end{restatable}
\begin{restatable}{theorem}{ApproxW}\thml{approx-w}
Let $G$ be a weighted, undirected graph with aspect ratio $\De$.
There is a randomized algorithm that w.h.p., outputs a $(1+\e)$-approximate Gomory-Hu Steiner tree and runs in $\tO(m)$ time plus calls to max-flow on instances with a total of $\tO(n\e\inv\log^2\De)$ vertices and $\tO(n\e\inv\log^2\De)$ edges. Assuming polynomial aspect ratio and using the $\tO(m+n^{1.5})$ time max-flow algorithm of ???, the algorithm runs in $\tO(m+n^{1.5})$ time.
\end{restatable}

Our algorithms use the following subroutine, which we call Cut Threshold \alert{better name?}, which may have further applications on their own:

\begin{restatable}{theorem}{Thr}\thml{thr}
Let $G=(V,E)$ be a weighted, undirected graph, let $s\in V$, and let $\la\ge0$ be a parameter. There is an algorithm that outputs all vertices $v\in V$ with $\mincut(s,v)\le\la$, and runs in $\tO(m)$ time plus $\pl(n)$ calls to max-flow on $O(n)$-vertex, $O(m)$-edge graphs.
\end{restatable}

In particular, \thm{thr} implies an algorithm for approximate single-source min-cut that is faster than running approximate min-cut separately for each vertex.

\begin{restatable}{theorem}{SSMC}\thml{ssmc}
Let $G$ be a weighted, undirected graph with aspect ratio $\De$, and let $s\in V$. There is an algorithm that outputs, for each vertex $v\in V\sm\{s\}$, a $(1+\e)$-approximation of $\mincut(s,v)$, and runs in $\tO(m\log\De)$ time plus $\pl(n)\log\De$ calls to max-flow on $O(n)$-vertex, $O(m)$-edge graphs.
\end{restatable}

}

